Session Logical Relations for Noninterference

Information flow control type systems statically restrict the propagation of sensitive data to ensure end-to-end confidentiality. The property to be shown is noninterference, asserting that an attacker cannot infer any secrets from made observations. Session types delimit the kinds of observations that can be made along a communication channel by imposing a protocol of message exchange. These protocols govern the exchange along a single channel and leave unconstrained the propagation along adjacent channels. This paper contributes an information flow control type system for linear session types. The type system stands in close correspondence with intuitionistic linear logic. Intuitionistic linear logic typing ensures that process configurations form a tree such that client processes are parent nodes and provider processes child nodes. To control the propagation of secret messages, the type system is enriched with secrecy levels and arranges these levels to be aligned with the configuration tree. Two levels are associated with every process: the maximal secrecy denoting the process' security clearance and the running secrecy denoting the highest level of secret information obtained so far. The computational semantics naturally stratifies process configurations such that higher-secrecy processes are parents of lower-secrecy ones, an invariant enforced by typing. Noninterference is stated in terms of a logical relation that is indexed by the secrecy-level-enriched session types. The logical relation contributes a novel development of logical relations for session typed languages as it considers open configurations, allowing for more nuanced equivalence statement.

==> more_mot_example.tex <==
\section*{Indirect Flow via Send}

\begin{center}
\begin{small}
\begin{minipage}[t]{\textwidth}
\begin{tabbing}
$x_1{:} \&\{\mi{tok}_i{:}1\}_{i \in \{1 \dots n\}}\maxsec{[\mb{guest}]},  u{:}\,\&\{\mathit{s}{:}\m{account}, \mathit{f}{:}1\}\maxsec{[\mb{alice}]} \vdash$ \\
$\m{SneakyaAuth} :: x{:}\m{auth}\maxsec{[\mb{alice}]}$ \\
$x \leftarrow \m{SneakyaAuth}\leftarrow u, x_1 = ($ \\
\quad \= $\mb{case} \, x \, ($\= $\mathit{tok}_j \Rightarrow$ \=$x.\mathit{succ};u.\mathit{s}; x_1.\mathit{tok}_{j};$
\comment{// insecure send} \\
\> \> \>$\mb{send}\, u\, x ; \mb{wait}\, x_1; \mb{close}\,x$ \\
\> \> $\mid \mathit{tok}_{i \neq j} \Rightarrow$ \=$x.\mathit{fail}; u.\mathit{f}; x_1.\mathit{tok}_{i};$
\comment{// insecure send} \\
\> \> \> $\mb{wait}\, u; \mb{wait}\, x_1; \mb{close}\, x ))\runsec{@\mb{alice}}$
\end{tabbing}
\end{minipage}
\end{small}
\end{center}

alternative version

\begin{center}
\begin{small}
\begin{minipage}[t]{\textwidth}
\begin{tabbing}
$x_1{:} \&\{s{:}\&\{\mi{tok}_i{:}1\}_{i  \in \{1 \dots n\}}, f{:} 1\}\maxsec{[\mb{guest}]},$ \\
$u{:}\,\&\{\mathit{s}{:}\m{account}, \mathit{f}{:}1\}\maxsec{[\mb{alice}]} \vdash \m{SneakyaAuth} :: x{:}\m{auth}\maxsec{[\mb{alice}]}$ \\
$x \leftarrow \m{SneakyaAuth}\leftarrow u, x_1 = ($ \\
\quad \= $\mb{case} \, x \, ($\= $\mathit{tok}_j \Rightarrow$ \=$x.\mathit{succ};u.\mathit{s}; x_1.s; x_1.\mathit{tok}_{j};$
\comment{// insecure send} \\
\> \> \>$\mb{send}\, u\, x ; \mb{wait}\, x_1; \mb{close}\,x$ \\
\> \> $\mid \mathit{tok}_{i \neq j} \Rightarrow$ \=$x.\mathit{fail}; u.\mathit{f}; x_1.f;$
\comment{// insecure send} \\
\> \> \> $\mb{wait}\, u; \mb{wait}\, x_1; \mb{close}\, x ))\runsec{@\mb{alice}}$
\end{tabbing}
\end{minipage}
\end{small}
\end{center}

\section*{Indirect Flow via Cut}

For example, consider the below process
definition $\m{SneakyaAuth}$ that not only authenticates Alice but also indirectly leaks
information about Alice's authorization token to the adversary $x_1$ via spawning of processes
$\m{S}_j$ and $\m{F}$.

\begin{center}
\begin{small}
\begin{minipage}[t]{\textwidth}
\begin{tabbing}
$x_1{:} \&\{s{:}\&\{\mi{tok}_i{:}1\}_{i  \in \{1 \dots n\}}, f{:} 1\}\maxsec{[\mb{guest}]},$ \\
$u{:}\,\&\{\mathit{s}{:}\m{account}, \mathit{f}{:}1\}\maxsec{[\mb{alice}]} \vdash \m{SneakyaAuth} :: x{:}\m{auth}\maxsec{[\mb{alice}]}$ \\
$x \leftarrow \m{SneakyaAuth}\leftarrow u, x_1 = ($ \\
\quad \= $\mb{case} \, x \, ($\= $\mathit{tok}_j \Rightarrow$ \=$x.\mathit{succ};u.\mathit{s}; z_1 \leftarrow S_j \leftarrow x_1;$
\comment{// insecure spawn} \\
\> \> \>$\mb{send}\, u\, x ; \mb{wait}\, z_1; \mb{close}\,x$ \\
\> \> $\mid \mathit{tok}_{i \neq j} \Rightarrow$ \=$x.\mathit{fail}; u.\mathit{f}; z_1 \leftarrow F \leftarrow x_1;$
\comment{// insecure spawn} \\
\> \> \> $\mb{wait}\, u; \mb{wait}\, z_1; \mb{close}\, x ))\runsec{@\mb{alice}}$
\end{tabbing}
\end{minipage}
\end{small}
\end{center}

\noindent The processes $\m{S}_i$ and $\m{F}$ are defined below, where $\m{S}_i$ means that we
have a corresponding process definition for each authorization token in $\m{auth}$, recording
the choice of that very token.

\begin{center}
\begin{small}
\begin{minipage}[t]{\textwidth}
\begin{tabbing}
$\&\{s{:}\&\{\mi{tok}_i{:}1\}_{i  \in \{1 \dots n\}}, f{:} 1\}\maxsec{[\mb{guest}]} \vdash \m{S}_i :: z_1{:}1\maxsec{[\mb{alice}]}$ \\
$z_1 \leftarrow \m{S}_i\leftarrow x_1 = (x_1.s;x_1.\mathit{tok}_i; \mb{wait}\, x_1; \mb{close}\, z_1)\runsec{@\mb{guest}}$
\end{tabbing}
\end{minipage}
\end{small}
\end{center}

\begin{center}
\begin{small}
\begin{minipage}[t]{\textwidth}
\begin{tabbing}
$\&\{s{:}\&\{\mi{tok}_i{:}1\}_{i  \in \{1 \dots n\}}, f{:} 1\}\maxsec{[\mb{guest}]} \vdash \m{F} :: z_1{:}1\maxsec{[\mb{alice}]}$ \\
$z_1 \leftarrow \m{F}\leftarrow x_1 = (x_1.f; \mb{wait}\, x_1; \mb{close}\, z_1)\runsec{@\mb{guest}}$
\end{tabbing}
\end{minipage}
\end{small}
\end{center}

\noindent Even though the process definitions $\m{S}_i$ and $\m{F}$ are secure on their own,
the spawning of these processes in $\m{SneakyaAuth}$ is not secure because it occurs in a context
where information about Alice's authorization token has been obtained.

Like $\m{LeakyBank}$, $\m{SneakyaAuth}$ is not a well-typed $\lang$ process definition.  A
$\m{SneakyaAuth}$ process is spawned at running secrecy $\runsec{@\mb{alice}}$ to guard the
process' knowledge of Alice's authorization token.  To rule out indirect flows, the $\lang$ type system
requires any process to be spawned at at least the spawning process' running secrecy, which
would require the processes $\m{S}_i$ and $\m{F}$ to be spawned at running secrecy
$\runsec{@\mb{alice}}$, not $\runsec{@\mb{guest}}$.

==> tmp.tex <==
any two runs of a well-typed $\lang$ program emit the same messages
observable to an adversary

% FROM TYPE SYSTEM

%\[\begin{array}{cl}
 %   A::= &\oplus\{\ell:A\}_{\ell \in L} \mid \&\{\ell:A\}_{\ell \in L} \mid A \otimes A \mid A \multimap A \mid 1 
%\end{array}\]



%The grammar to define processes is as follows:
%Process terms with generations and secrecy labels.
%{\small{
%\[\begin{array}{ll}
%P,Q ::= &\\   
 %  { y_\alpha^c \leftarrow x_\beta^c} & \m{fwd}\\
  % \mid  ( x^d \leftarrow P_{x^d}@c ; Q_{x^d}) & \m{cut}^{x} \\
 %\mid \mathbf{close}\, x_\alpha^c \mid \mathbf{wait}\,x_\alpha^c;Q& 1\\
 %\mid x_\alpha^{c}.k; P  \mid \mathbf{case}\, x_\alpha^{c}(\ell \Rightarrow Q_{\ell})_{\ell \in L}& \& \{\ell{:}A_\ell\}_{\ell \in L}, \oplus \{\ell{:}A_\ell\}_{\ell \in L}  \\
%\mid \mathbf{send}\,x_\alpha^{c}y_\beta^{d}; P \mid y^{\omega} \leftarrow \mathbf{recv}\,x_\alpha^{c};P & A\otimes B,\, A \multimap B
%\end{array}\]}}

Notes on logical relation:

Capitalization
